A Composable Dynamic Sparse Dataflow Architecture for Efficient Event-based Vision Processing on FPGA

Event-based vision represents a paradigm shift in how vision information is captured and processed. By only responding to dynamic intensity changes in the scene, event-based sensing produces far less data than conventional frame-based cameras, promising to springboard a new generation of high-speed, low-power machines for edge intelligence. However, processing such dynamically sparse input originated from event cameras efficiently in real time, particularly with complex deep neural networks (DNN), remains a formidable challenge. Existing solutions that employ GPUs and other frame-based DNN accelerators often struggle to efficiently process the dynamically sparse event data, missing the opportunities to improve processing efficiency with sparse data. To address this, we propose ESDA, a composable dynamic sparse dataflow architecture that allows customized DNN accelerators to be constructed rapidly on FPGAs for event-based vision tasks. ESDA is a modular system that is composed of a set of parametrizable modules for each network layer type. These modules share a uniform sparse token-feature interface and can be connected easily to compose an all-on-chip dataflow accelerator on FPGA for each network model. To fully exploit the intrinsic sparsity in event data, ESDA incorporates the use of submanifold sparse convolutions that largely enhance the activation sparsity throughout the layers while simplifying hardware implementation. Finally, a network architecture and hardware implementation co-optimizing framework that allows tradeoffs between accuracy and performance is also presented. Experimental results demonstrate that when compared with existing GPU and hardware-accelerated solutions, ESDA achieves substantial speedup and improvement in energy efficiency across different applications, and it allows much wider design space for real-world deployments.

==> 01-intro_gyz.tex <==
\section{Introduction}

Event-based vision systems are bio-inspired systems that represent a paradigm shift from conventional frame-based vision systems~\cite{event-based-vision}. 
It aims to overcome the limitations of conventional vision systems by striving for intrinsic efficiency, low power consumption, and high-speed processing in visual perception and analysis. While Neuromorphic accelerators \cite{truenorth_chip, loihi, braindrop, SpiNNaker} that typically due with Spiking Neural Networks (SNNs) have been a natural hardware backend for event cameras,
recent breakthroughs in deep learning algorithms~\cite{deeplearning} have significantly enhanced the performance of event-based vision in various demanding tasks. For example, the state-of-the-art event-based object classification~\cite{asynet, mlp_repre, n_imagenet, tore_class, EvT}, object detection~\cite{onemega_detection, detection23, asydetect, detection_fusing}, object tracking~\cite{tracking_1, tracking_2, tracking3} optical flow~\cite{of_net1, of3, ev_flownet, of_tip, of_secret}, stereo~\cite{stereo1, stereo2, nam2022stereo, stereo3}, reconstruction~\cite{recons0, recons1, recons2} and etc, heavily utilize deep learning model as a powerful tool for extracting meaningful features and performing accurate analysis ~\cite{deep_event_survey}. 

However, deploying event-based vision systems with deep learning models in near-sensor or edge computing context still poses great challenges. 
The energy efficiency and high-speed promises of the event-based paradigm have yet to be realized in practice. 
On the one hand, unlike conventional frame-based inputs that are 2D dense matrix, off-the-shelf GPU platforms and other dense accelerators can not fully exploit the sparsity in event-based inputs. Utilizing these hardware architectures can result in high energy consumption stemming from the wasted computation.
On the other hand, prior sparse DNN accelerators or sparse tensor accelerators operating at the layer or matrix multiplication levels can also suffer from significant latency and energy overhead brought by the frequent I/O of weight and intermediate results. 
As a result, developing a domain-specific architecture that can effectively leverage the intrinsic sparsity in event-based data while achieving low latency and energy consumption emerges as a critical research problem. 

To address these challenges, we introduce \aname, a system based on FPGA that can efficiently accelerate \textbf{E}vent-based vision processing with a composable dynamic \textbf{Spa}rse \textbf{D}ataflow \textbf{A}rchitecture. In a nutshell, 
\aname belongs to the family of the all-on-chip dataflow or streaming FPGA DNN accelerator that pipelines all the layers of a model in a single FPGA device. Employing the all-on-chip dataflow architecture is a key design choice towards low latency and power consumption by minimizing the off-chip communication of weight and activation. However, in contrast to prior dataflow architectures that handle dense frame-based input, \aname embraces a sparse dataflow approach, exclusively streaming the spatially sparse features from the event-based input. The advantages of the sparse dataflow approach are further magnified through the integration of submanifold sparse convolution~\cite{submanifold} at the algorithmic level. Submanifold convolution can effectively maintain high spatial sparsity of feature activations of the models by constraining the spatial activation locations.  

\begin{figure*}[t]
    \includegraphics[width=1\linewidth]{fig/new_event_plot.pdf}
    \centering
    \caption{Working principle of event camera. The event camera only captures the light intensity change as spiking events in AER format ([x, y, ±1, timestamp]). This figure shows a recording sample from DvsGesture dataset where a man is rotating his left arm counter-clockwise. Due to the dynamic nature of event camera, only the motions of the man are captured. For high-level vision tasks like object recognition, a certain amount of events are usually grouped to form a 2D representation as DNN input.}     
    \label{fig:event_principle}
\end{figure*}

The proposed \aname framework is well-suited for FPGA implementation. Leveraging the FPGA's reconfigurability, it can seamlessly deploy different DNN models by spatially composing different sparse dataflow modules on the programmable fabric. Each dataflow template in \aname is highly modular and shares a unified sparse token-feature interface. To strike a balance between accuracy and hardware efficiency, we also develop a series of model architecture and hardware co-optimization frameworks that can take advantage of the sparsity statistics from each event-based vision task or dataset. 
To this end, the main contribution of this work can be summary as:

\begin{itemize}
\item We proposed a novel composable sparse dataflow architecture for DNN inference in event-based vision, effectively harnessing sparsity within both algorithmic and architectural perspectives. 
\item We implemented \aname on embedded FPGA platforms and established a set of sparsity-aware co-optimization flow, enabling the customization of DNN accelerators for each specific application or dataset.
\item We showcased a substantial end-to-end hardware speedup and energy-efficiency improvement through extensive evaluation on multiple event-based datasets.
\end{itemize}






In the next section, background and related work about neuromorphic vision systems and processing will first be provided. The detailed design of \aname will be discussed in \secref{sec:methodology}. Experiment results are shown in \secref{sec:evaluations} and we will conclude in \secref{sec:conclusion}.  

==> 03-method_old.tex <==
\section{Methodology} \label{sec:methodology}


\begin{figure*}[t]
    \includegraphics[width=\linewidth]{fig/architecture.pdf}
    \centering
    \caption{System diagram of \aname. An event camera captures light intensity changes as events and outputs as AER format, which encodes the location of the event, timestamps, and polarity of intensity changes ($[x,y,t,p]$). The left plot show two examples from the DvsGesture dataset. Each segment of event stream will first be sampled and constructed into a 2D feature and fed to \aname accelerator. The accelerator reads only the compressed feature and the bitmap that encodes non-zero pixels as `1's. The hardware then streams the feature and token pixel by pixel to the following convolutional engines. The last Pooling and FC iterate and aggregates global information and produce classification results.} 
    
    \label{fig:system}
\end{figure*}

\subsection{System Architecture of \aname}
\figref{fig:system} shows the overall system diagram for \aname. The left figure shows an example 3D plot of events in the spatial-temporal space. The sample comes from the DvsGesture dataset~\cite{dvsgesture}. Following the practice of many state-of-the-art algorithms, the events are sampled in a fixed time interval and constructed into some 2D feature before feeding into the neural network accelerator. Many previous research works have explored using different algorithms in the 2D representation, such as event histogram~\cite{histogram_and_autodrive}, time-surface~\cite{hots, hats}, or even learnable kernels~\cite{mlp_repre}, etc. It should be noted that the 2D feature construction algorithm is independent of our hardware accelerator, meaning our hardware can be combined with any pre-processing algorithm as long as it produces reasonable sparsity. Users can also implement the 2D feature construction process as part of the accelerator to speed up end-to-end performances. 
To simplify hardware testing flow and maintain flexibility, our current hardware implementation directly reads 2D sparse features with a binary bitmap that indicates non-zero pixel locations. Using the sparsity information from the bitmap, an input Tokenizer will generate two streams: a feature stream and a token stream to the downstream DNN modules. Each token is written as a $[.x, .y, .end]$ struct where $[.x, .y]$ denotes the current pixel locations, and $.end$ flags whether it's the last element in a sample. The token stream and features stream are synchronized, meaning that each token $[.x, .y, .end]$ corresponds to all the features $[f_1, f_2, ..., f_c]$ at location $[.x, .y]$ with $c$ being the number of channels. 


The dataflow accelerator is fully pipelined on-chip across all the layers in a model by cascading all the modules using dataflow stream FIFOs. Different from standard inter-layer pipeline architecture that only has feature streams, \aname introduces an additional token stream to help control the sparse convolution in different modules. 
The dataflow generally follows standard sliding window algorithms, while it only iterates on non-zero spatial locations. 
\figref{fig:blocks} shows the major building blocks in \aname. Each dataflow module can operate autonomously during runtime, using input tokens and features locally to compute the output token and features. 
This design ensures that different modules in the dataflow path can be fully pipelined and operator on different spatial locations (tokens) without global-wise control and synchronization. The weights of different layers are treated as static on-chip in local buffers for each layer. 

\figref{fig:timing} shows an example timing diagram of the dynamic sparse dataflow with two consecutive $1\times1$, $3\times3$ and $1\times1$ convolution blocks. The strides of the two $3\times3$ convolution layers are 1 and 2 respectively. The channel dimension is omitted in the figure for simplicity. The above timing diagram in \figref{fig:timing} shows how different layers can overlap the computation on sparse input in the pipeline. The snapshots below showcase the computation status for different layers at the time slot marked in green. 
For $1\times1$ convolution, it involves only local updates of features and iterates through each non-zero location one by one. In contrast, $3\times 3$ convolution uses a Sparse Line Buffer design to control the dataflow and resolve dependencies, allowing it to perform weighted summation over neighborhood non-zero features efficiently. 
This figure provides an overview of the sparse dataflow, offering insight into the pipelined computation. In the next section, we will explore the  design details of these modules, demonstrating how they leverage the dynamic sparsity of event-based data.

\begin{figure}[t]
    \includegraphics[width=0.9\linewidth]{fig/timing_diagram.pdf}
    \centering
    \caption{Example timing diagram of the sparse dataflow. The example demonstrates two consecutive convolution blocks ($1\times1$, $3\times 3$ and $1\times1$). The strides of $3\times 3$ layers are 1 and 2 respectively. The sparse dataflow only streams features at non-zero spatial locations. H and W are the height and width of the input feature
    and for simplicity, the channel dimension is omitted. The dependencies that are dynamically handled by the Sparse Line Buffer using the logic in \eqnref{eq:elb}. }
    \label{fig:timing}
\end{figure}

\subsection{Modular Building Blocks in \aname}
\label{subsec:blocks}


\begin{figure*}[t]
    \includegraphics[width=1\linewidth]{fig/blocksv2.pdf}
    \centering
    \caption{Modular building blocks of \aname.}
    \label{fig:blocks}
\end{figure*}

\subsubsection{$1\times 1$ Convolution Module}
Since $1\times 1$ convolution computes each output feature locally for each non-zero pixel, the input and output token can simply be relayed. \figref{fig:blocks}a shows the hardware diagram. The features at the current location $[.x, .y]$ are first read into an input feature buffer and then multiplied with the weights in the static buffer. As a result, the computation can be implemented as a Matrix-Vector multiplication using a PE array as illustrated in \figref{fig:blocks}a.
Note that the element-wise batch norm is folded into the convolutional weights, and the activation function is omitted from the diagram for simplicity.  
The final output features are packed into streams as output. As a modular hardware template, the configurations of the PE array (the parallelism factors on channel dimensions) are exposed as hardware design parameters.  

\subsubsection{$k\times k$ Convolution Module ($k>1$)}
Different from $1\times1$ convolution that can directly operate on non-zeros, when the convolution kernel size $k$ is larger than 1, the computation requires the summation over neighborhood features in the sliding window. In \aname, $k\times k$ convolution is done by combining a Sparse Line Buffer module and a convolution computation module. Different line buffer designs are needed depending on the convolution stride (usually 1 or 2), while the computation engine remains the same. 
To leverage the sparsity within each $k\times k$ window, an additional kernel offset stream is used when streaming data from line buffer to compute engine. \figref{fig:blocks}b shows the diagram of $3\times 3$ depthwise convolution module, which is widely used in many mobile networks~\cite{mobilenetv2, mnasnet, efficientnet}. 
For each non-zero output location marked by the current token register, a variable number of features can be read into the module, which is synchronized by the kernel offset streams. The kernel offset denotes the relative spatial locations of the current input feature in the sliding window and selects the correct weights to multiply. After performing the weighted sum for all non-zero kernel offsets, the final summation will be read out as feature streams. 
Even though \figref{fig:blocks}b only shows the diagram of depth-wise $3\times3$ convolution units, other types of convolution with different channel grouping numbers only differ in the PE organization part. 
Similar to $1\times 1$ convolution module, the hardware template also incorporates the channel dimension parallelism factor as an optimization variable for design space exploration.


\subsubsection{Sparse Line Buffer with Stride Equals 1}
% The concept of Sparse Line Buffer (SLB) is extended from the Elastic Line Buffer design proposed in DPACS~\cite{dpcas}. In this work, we extend the original Elastic Line Buffer design to fully support submanifold sparse convolution with both strides of 1 and 2. 
The Sparse Line Buffer (SLB) is a key module to achieve submanifold sparse convolution on large kernels. 
It mainly comprises a $k$ lines data buffer ($k$ being the kernel size), a token FIFO, and a small bitmap to record current non-zero spatial locations in the buffer. 
When stride equals 1, the submanifold convolution algorithm enforces the input and output non-zero locations to be unchanged as shown in \figref{fig:submanifold}. As a result, a simple token FIFO is used to set up a queue for output tokens.  
Due to the deterministic streaming order of the sliding window algorithm (from left to right, top to bottom shown in \figref{fig:timing}), we can leverage the token FIFO's head and tail tokens to control the read and write logic of SLB. 
The tail token serves as a clue to determine whether the current buffer contains all the data required for the data window center at the head token. If so, the head token can be popped out, and the corresponding features can be output for computation. 
On the other hand, new tokens and features can be read into the SLB if the new token points to locations that still lie within the current buffered rows. 
The control signals ready $r$ and valid $v$ can then be written as: 
\begin{equation}
\small
\begin{split}
    u&=(k-1)/2\\
    v&=((t.x-h.x\geq u) \wedge (t.y-h.y\geq u))\vee (t.y-h.y\geq u + 1)\\
    r&= (t.y-h.y\leq u)
\end{split}
\label{eq:elb}
\end{equation}
where $h,t$ stands for head and tail tokens. $u$ is the radius of the kernel. 
This design is deadlock-free because when a new token arrives outside the current buffered rows, it implies that tokens in upper rows ($t.y - u - 1$) are all valid to output. Consequently, these tokens will be popped out one by one, and buffers will be clean to allow continuous data flow without any deadlocks.

As mentioned earlier, kernel sparsity can also exist for each output $k\times k$ window. To avoid unnecessary computation for those zero pixels, only non-zero features are fed into the $k\times k$ convolution module. The kernel offset stream is used to denote each non-zero location within the $k\times k$ window. This information is obtained by querying the bitmap of the buffer, which marks whether a spatial location in the buffer is non-zero or not.
\figref{fig:blocks}d shows an example diagram of an SLB for $3\times 3$ convolution. The kernel offset stream $[2,4, 6, 8]$ corresponds with the non-zero features.    


\subsubsection{Sparse Line Buffer with Stride Equals 2}
Convolution with its stride equals two will downsample the image in the spatial dimension. 
As illustrated in \figref{fig:submanifold}, when the stride equals 2, the sparse convolution requires recalculating the non-zero coordinates (tokens). 
For each $2\times 2$ stride grid, if it contains any non-zero pixels, it will be considered to be a non-zero output. 
To accommodate this scenario, the Sparse Line Buffer module with strides equal to 2 (SLB s2) uses two token FIFOs to buffer tokens in even and odd rows, respectively. A Token Merge unit is positioned at the head of the FIFOs to generate new valid output tokens. 
Similar to the case with stride equals 1, the tail token can assist in determining whether the latest new output token has sufficient data for the $3\time 3$ window to be output. The control logic is similar to \eqnref{eq:elb}, with the head token being replaced by the newly generated output token. 

In \figref{fig:blocks}e, an example of a $3\times 3$ SLB S2 is illustrated, where the blue and green locations within the $2\times 2$ stride grid contribute to a valid output location. When a valid output is triggered, the token merge units will pop all the tokens from both token FIFOs in the stride grid (blue and green in the example).
The SLB then streams out the new output token with corresponding features and kernel offsets for downstream computation. 


\subsubsection{Pooling and FC Module}
For the classification tasks, the network typically includes a global pooling followed by a fully connected layer to generate predictions. In the sparse dataflow of \aname, the global pooling layer will iterate through all the non-zero tokens until it encounter an \emph{end} flag. Depending on the pooling algorithm (max or average), the feature are aggregated into a single vector and fed into the final linear classifier layer. \figref{fig:blocks}c shows an example of global average pooling with a linear classifier. 

\subsubsection{Chaining Modules into a Block}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{fig/conv_blocks.pdf}
    \centering
    \caption{Forming convolution blocks MBConv by cascading modules. T, K, and F stand for token, kernel offset, and feature streams.}
    \label{fig:convblock}
\end{figure}

Many widely adopted DNN models are built upon small convolution layers and may incorporate some residual connections~\cite{resnet}. Thanks to the unified and autonomous dynamic sparse behavior of all the modules in \aname, building these blocks by chaining the dataflow streams between modules is straightforward. \figref{fig:convblock} shows two examples of building the mobile inverted residual blocks MBConv used in \aname. The MBConv blocks commonly employed in networks like MobileNetV2~\cite{mobilenetv2}, EfficientNet~\cite{efficientnet}, MnasNet~\cite{mnasnet}, etc.  Although this work mainly uses MBConv blocks in the experiments, similar approaches can be applied to other models like ResNet~\cite{resnet}, ShuffleNet~\cite{shufflenet}, etc. 

\figref{fig:convblock}a shows the case of having an identity shortcut in a block with all the layer strides being 1. Due to the usage of submanifold convolution, the input and output tokens are identical for all the layers. Thus, the input feature stream can simply be forked into two streams with one for the residual functional layers and the other one for the identity shortcut. 
The shortcut branch features are buffered in a FIFO and added at the output of the last $1\times 1$ convolution layer. For the MBConv block with stride equals 2, the tokens are updated in the SLB s2 module, where the downsampling of the image happens.

% \subsection{Dynamic Activation Pruning}
% \aname also incorporates a dynamic activation pruning mechanism in the framework. As mentioned in previous sections, the proposed dynamic activation pruning method aims to improve the runtime sparsity of data while achieving a similar effect of denoising. As the dataflow in \aname typically targets spatial sparsity, the dynamic pruning algorithm also applies to the spatial dimension. In other words, for each non-zero location, a trainable pruning module will determine whether to remove all the features at this location during runtime. 

% Motivated by other dynamic spatial pruning algorithms in point cloud ~\cite{point_pruning, point_pruning2} and frame-based vision~\cite{dyspatial, dpcas}, we design the dynamic pruning module to make pruning decisions based on the summation of activations. 
% Specifically, if the summation of the features across all the channels at a non-zero location is lower than a trainable threshold, the features will be pruned (change into zeros). 
% From the dataflow perspective, tokens and features will be dropped out of the pipelined if the pruning decisions are made.   
% The threshold $\theta$ is trained using momentum update. 
% Each pruning module has a pre-defined targeted pruning ratio $r$, e.g. 10\%.  
% During training, it first calculates the exact threshold $\theta_r$ that achieves the pruning ratio $r$ for every mini-batch of input.  
% Then the threshold $\theta$ is updated using:
% \begin{equation}
%     \theta_{new} = (1-m)\times \theta_{old} + m \times \theta_r
% \end{equation}
% where $m$ is the momentum.

% The dynamic activation pruning module is implemented at the convolution block level. 
% As depicted in \figref{fig:convblock}, the hardware diagram showcases the MBConv blocks with the pruning module placed at the beginning of the block. 
% Since the residual connection in a convolution block leads to two branches, if to place the pruning unit within the residual function branch, it's difficult to synchronize the pruning decision in the identity shortcut branch. This can easily result in dataflow deadlock during runtime. As a result, positioning the pruning unit at the beginning of the block simplifies the hardware implementation.   

% \figref{fig:blocks}f shows the micro-architecture of the hardware pruning module. The input features at the current token location are first buffered and fed to an adder tree to calculate the summation across all the channels. If the summation is higher than the trainable threshold, the features will be read out from the buffer and stream to the next module. Otherwise, both tokens and features will be discarded. 

\begin{figure}[t]
    \includegraphics[width=\linewidth]{fig/eda.pdf}
    \centering
    \caption{Design flow of \aname.}
    \label{fig:eda}
\end{figure}

\subsection{Design Automation in \aname}


Current \aname targets edge FPGAs platforms. To facilitate design closures and find feasible hardware and software solutions that satisfy the resource/application constraints, we develop several design space exploration and optimization flows. 

\subsubsection{Sparsity-awared Hardware Optimization}
In a dataflow accelerator, the throughput is usually bounded by the slowest in the pipeline. Thus, finding load-balanced hardware resource configurations for different modules is critical. 
To automatically obtain optimal hardware configuration of the proposed sparse dataflow architecture, we develop a static optimization strategy by using application-wise sparsity statistics. In other words, for each application/dataset, we collect the spatial and kernel sparsity ratio ($S_{s}$ and $S_{k}$) from all the samples in the dataset and use them to search for the optimal mapping of hardware resources. \figref{fig:eda} shows the overall diagram of our optimization flow. For each convolution module, we estimate averaged latency and resource utilization using the sparsity statistics. 
Take the depthwise $3\times3$ convolution as an example. The latency, the number of Block RAM (BRAM), and the DSP consumption on an FPGA can be estimated as:
\begin{equation}
\begin{split}
    lat &= (H \times W \times S_s)\times (9\times S_k) \times (C/PF) \\ 
    bram &= \lceil(B \times 9 \times C) / 16 \text{K} / PF\rceil \times PF\\
    dsp &= PF
\end{split}
\end{equation}
where $H,W$ is the output height and width in the current layer, $C$ is the number of channels, and $PF$ is the hardware parallelism factor. $B$ is the bitwidth of the quantized weight and a BRAM can store 16 Kb data. 
The $(H \times W \times S_s)$ term reflects the averaged number of iterations on the spatial dimension of this layer and $(9\times S_k) \times (C/PF)$ estimates the averaged cycles needed for computing an output. While the weight buffer needed to be partitioned to satisfy the on-chip bandwidth requirement determined by the parallelism factor $PF$. 
Using similar approaches, we can formulate the latency and resource utilization for other modules. Since we pipeline all the layers in the model, the theoretical throughput can be estimated by the maximum latency in all layers. 
With that, the overall hardware optimization problem can be written as:
\begin{equation}
    \begin{split}
        \min \quad  lat& \\
        \text{s.t.}\quad  lat_i &\leq lat,\quad i \text{ in all layers} \\
                         \sum_i r_{ij}& \leq R_j,\quad i\text{  in all layers, j in [BRAM, DSP] }
    \end{split}
\end{equation}
where $r_{ij}$ means resource used in layer $i$. $R$ is the total resource of each kind available. The current framework mainly concerns BRAM and DSP resources on FPGA. The proposed optimization program will be solved by open-sourced mixed integer programming solver. 
% The optimization program will be solved using the open-sourced Mixed-integer Geometric Programming framework developed in \cite{agna}. The optimizer can search for the close-to-optimal hardware configuration for each module and generate the final FPGA implementation. \XX{move AGNA to experiment setup}





\begin{figure*}[t]
    \includegraphics[width=\linewidth]{fig/kernel_sparsity.pdf}
    \centering
    \caption{
    X label with 8x8, etc. X label spatial resolution. Y label, Spatial Sparsity (\% of non-zeros). 
    }
    \label{fig:sparsity statistic}
\end{figure*}


\subsubsection{Neural Architecture Search}
\label{subsubsec:nas}
For some application scenarios with tight resource or power constraints, deploying larger models like ResNet might not be feasible. Many previous works have explored integrating Neural Architecture Search into the deployment process to facilitate the model performances while satisfying the hardware constraints. 
As shown in \figref{fig:eda}, our hardware optimizer can return the latency and resource utilization as the feedback information in a NAS framework. 

As a proof-of-concept experiment, we develop a simple two-step neural architecture search framework. The software first randomly samples a pool of neural architectures built upon the MBConv convolution block. The search space comprises different: 1) number of blocks; 2) types of blocks 2) number of channels in each layer. While the total downsample ratio of each dataset remains fixed.
The sampled models are fed into the MIGP optimizer along with the sparsity statistic. The hardware optimizer will search for the optimal hardware mapping of each model and estimate the performance. However, some large models might not be feasible to be implemented on small devices. Those models are subsequently filtered out automatically through this framework. The searching time for each model only takes around seconds to minutes. After obtaining all the  results, the software then chooses the top-k feasible models with the highest throughput and process to the training pipeline. 
In this way, we choose the one that best satisfies our application constraints and trade-off between accuracy and hardware performance. 
It should be noted that our current simple NAS algorithm does not integrate any sophisticated reinforcement learning or other meta-learning algorithms. However, such integration is entirely feasible and can be a promising avenue for future exploration.


